Where2Act: From Pixels to Actions for Articulated 3D Objects

One of the fundamental goals of visual perception is to allow agents to meaningfully interact with their environment. In this paper, we take a step towards that long-term goal -- we extract highly localized actionable information related to elementary actions such as pushing or pulling for articulated objects with movable parts. For example, given a drawer, our network predicts that applying a pulling force on the handle opens the drawer. We propose, discuss, and evaluate novel network architectures that given image and depth data, predict the set of actions possible at each pixel, and the regions over articulated parts that are likely to move under the force. We propose a learning-from-interaction framework with an online data sampling strategy that allows us to train the network in simulation (SAPIEN) and generalizes across categories. Check the website for code and data release: https://cs.stanford.edu/~kaichun/where2act/

==> tabs/fulltable.tex <==
\begin{table*}[t]
  \centering
    \setlength{\tabcolsep}{5pt}
  \renewcommand\arraystretch{0.5}
  \small
\begin{tabular}{@{}llcccccc@{}}
\toprule
&& \textsf{\footnotesize Precision (\%)} & \textsf{\footnotesize Recall (\%)} & \textsf{\footnotesize F-score (\%)} & \textsf{\footnotesize False-Acc (\%)} & \textsf{\footnotesize Avg-Acc (\%)} & \textsf{\footnotesize Sample-Succ (\%)}  \\
\midrule
\multirow{5}{*}{pushing}
& B-Random &  6.83 / 3.99 & 50.00 / 50.00 & 12.02 / 7.40 & 50.00 / 50.00 & 50.00 / 50.00 & 6.80 / 3.79 \\
& B-Normal & 19.75 / 9.89 & 83.48 / 71.63 & 31.94 / 17.39 & 75.12 / 72.87 & 79.30 / 72.25 & 21.72 / 11.57 \\
& B-PCPNet & 19.93 / 10.34 & 81.33 / 76.47 & 32.01 / 18.21 & 76.03 / 72.41 & 78.68 / 74.44 & 18.04 / 9.15 \\
& 3D-Ablated & 26.29 / 15.14 & \textbf{88.46} / \textbf{84.08} & 40.54 / 25.66 & 81.82 / 80.40 & 85.14 / \textbf{82.24} & 25.18 / 11.76 \\
& 3D-ours & \textbf{29.12} / \textbf{16.47} & 88.01 / 69.20 & \textbf{43.76} / \textbf{26.61} & \textbf{84.29} / \textbf{85.41} & \textbf{86.15} / 77.31 & \textbf{28.54} / \textbf{14.74} \\
& 2D-ours & 21.84 / 13.81 & 78.85 / 63.32 & 34.21 / 22.68 & 79.31 / 83.57 & 79.08 / 73.44 & 21.36 / 10.58 \\
\midrule
\multirow{5}{*}{pushing-up}
& B-Random & 2.59 / 1.71 & 50.00 / 50.00 & 4.92 / 3.31 & 50.00 / 50.00 & 50.00 / 50.00 & 2.70 / 1.62 \\
& B-Normal & 7.24 / 3.98 & 86.58 / 75.87 & 13.37 / 7.56 & 70.57 / 68.06 & 78.58 / 71.97 & 8.93 / 4.81 \\
& B-PCPNet & 8.33 / 3.98 & 79.92 / 65.42 & 15.08 / 7.50 & 76.65 / 72.45 & 78.29 / 68.93 & 8.09 / 4.86 \\
& 3D-Ablated & 11.94 / \textbf{6.26} & 87.87 / \textbf{76.14} & 21.03 / \textbf{11.57} & 82.80 / 80.11 & 85.34 / \textbf{78.12} & \textbf{12.88} / 6.43 \\
& 3D-ours & \textbf{12.33} / 6.11 & \textbf{87.97} / 66.49 & \textbf{21.64} / 11.20 & \textbf{83.41} / \textbf{82.19} & \textbf{85.69} / 74.34 & 12.06 / \textbf{6.56} \\
& 2D-ours & 8.50 / 4.73 & 78.83 / 53.08 & 15.35 / 8.69 & 77.49 / 81.36 & 78.16 / 67.22 & 8.70 / 5.76 \\
\midrule
\multirow{5}{*}{pushing-left}
& B-Random & 3.30 / 2.11 & 50.00 / 50.00 & 6.18 / 4.05 & 50.00 / 50.00 & 50.00 / 50.00 & 3.08 / 2.26 \\
& B-Normal & 10.40 / 5.76 & 84.95 / 77.02 & 18.52 / 10.72 & 75.05 / 72.86 & 80.00 / 74.94 & 11.59 / 5.72 \\
& B-PCPNet & 10.54 / 5.80 & 81.36 / 78.56 & 18.66 / 10.81 & 76.47 / 72.54 & 78.91 / 75.55 & 9.69 / 4.43 \\
& 3D-Ablated & 14.36 / 8.21 & \textbf{88.38} / \textbf{80.96} & 24.71 / 14.91 & 82.05 / 80.52 & \textbf{85.21} / \textbf{80.74} & 14.12 / 7.02 \\
& 3D-ours & \textbf{15.37} / \textbf{8.97} & 85.02 / 76.59 & \textbf{26.04} / \textbf{16.06} & \textbf{84.05} / \textbf{83.27} & 84.54 / 79.93 & \textbf{15.95} / \textbf{9.31} \\
& 2D-ours & 10.81 / 6.64 & 76.13 / 64.77 & 18.93 / 12.04 & 78.59 / 80.38 & 77.36 / 72.58 & 11.68 / 7.22 \\
\midrule
\multirow{5}{*}{pulling}
& B-Random & 1.16 / 1.65 & 50.00 / 50.00 & 2.26 / 3.19 & 50.00 / 50.00 & 50.00 / 50.00 & 1.07 / 1.55 \\
& B-Normal & 3.23 / 4.23 & 80.91 / 78.06 & 6.20 / 8.02 & 71.55 / 70.41 & 76.23 / 74.24 & 3.79 / 4.18 \\
& B-PCPNet & 3.77 / 4.52 & 77.97 / 81.18 & 7.19 / 8.57 & 76.65 / 71.34 & 77.31 / 76.26 & 4.15 / 3.71 \\
& 3D-Ablated & 5.45 / 6.49 & \textbf{90.31} / \textbf{88.37} & 10.28 / 12.09 & 81.63 / 78.69 & \textbf{85.97} / \textbf{83.53} & 5.62 / 5.87 \\
& 3D-ours & \textbf{5.84} / \textbf{6.96} & 87.65 / 86.33 & \textbf{10.95} / \textbf{12.88} & \textbf{83.43} / \textbf{80.70} & 85.54 / 83.51 & \textbf{7.51} / \textbf{7.85} \\
& 2D-ours & 3.68 / 4.80 & 79.20 / 70.74 & 7.04 / 8.98 & 75.71 / 76.51 & 77.46 / 73.62 & 4.07 / 4.70 \\
\midrule
\multirow{5}{*}{pulling-up}
& B-Random & 2.63 / 2.16 & 50.00 / 50.00 & 5.01 / 4.13 & 50.00 / 50.00 & 50.00 / 50.00 & 2.22 / 2.41 \\
& B-Normal & 7.44 / 5.02 & 82.42 / 73.66 & 13.64 / 9.40 & 72.24 / 69.29 & 77.33 / 71.48 & 8.67 / 6.08 \\
& B-PCPNet & 8.16 / 5.89 & 75.68 / 80.30 & 14.73 / 10.98 & 76.94 / 71.74 & 76.31 / 76.02 & 8.37 / 6.19 \\
& 3D-Ablated & 11.59 / 7.43 & \textbf{88.87} / \textbf{87.58} & 20.51 / 13.70 & 81.66 / 75.97 & \textbf{85.26} / \textbf{81.77} & 12.18 / 7.96 \\
& 3D-ours & \textbf{12.78} / \textbf{9.11} & 85.55 / 76.23 & \textbf{22.24} / \textbf{16.28} & \textbf{84.20} / \textbf{83.25} & 84.87 / 79.74 & \textbf{13.53} / \textbf{9.28} \\
& 2D-ours & 8.77 / 7.15 & 77.15 / 64.45 & 15.74 / 12.88 & 78.27 / 81.56 & 77.71 / 73.01 & 9.71 / 7.10 \\
\midrule
\multirow{5}{*}{pulling-left}
& B-Random & 3.10 / 2.17 & 50.00 / 50.00 & 5.83 / 4.16 & 50.00 / 50.00 & 50.00 / 50.00 & 3.06 / 2.31 \\
& B-Normal & 9.78 / 5.67 & 83.79 / 71.64 & 17.52 / 10.51 & 75.31 / 73.55 & 79.55 / 72.60 & 11.14 / 5.82 \\
& B-PCPNet & 10.74 / 5.97 & 78.30 / 69.94 & 18.89 / 11.00 & 79.20 / 75.54 & 78.75 / 72.74 & 9.12 / 5.19 \\
& 3D-Ablated & 13.46 / \textbf{8.28} & \textbf{89.53} / \textbf{84.22} & 23.41 / \textbf{15.07} & 81.62 / 79.28 & \textbf{85.57} / \textbf{81.75} & 14.23 / 6.81 \\
& 3D-ours & \textbf{14.85} / 8.05 & 83.62 / 71.86 & \textbf{25.22} / 14.49 & \textbf{84.68} / \textbf{81.79} & 84.15 / 76.82 & \textbf{14.25} / \textbf{7.10}   \\
& 2D-ours & 9.00 / 5.50 & 80.63 / 66.31 & 16.20 / 10.16 & 73.96 / 74.71 & 77.30 / 70.51 & 10.15 / 6.05 \\
\bottomrule
\end{tabular}
  \caption{\titlecap{Quantitative Evaluations and Comparisons.}{We compare our method to three baseline methods (\ie \textbf{B-Random}, \textbf{B-Normal} and \textbf{B-PCPNet}) and one ablated version of our method (\ie \textbf{3D-Ablated}), where we remove the online adaptive sampling. In each entry, we report the numbers evaluated over the testing shapes from training categories (before slash) and the testing shapes from the test categories (after slash). We use \textbf{3D-} and \textbf{2D-} to indicate the data input modalities. The baseline methods are not sensitive to the input kinds. We observe that \textbf{3D-ours} achieves the best performance over most metrics.}}
  \label{tab:results_full}
  \vspace{-4mm}
\end{table*}%

==> tex/intro_donotusethis.tex <==
\kaichun{comment}
\leo{comment}
\abhinav{comment}
\shubham{comment}
\mustafa{comment}
\eg \ie

\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{fig/teaser.pdf}
    \caption{\titlecap{The Proposed Where2Act Task.}{Given as input as articulated 3D object, we learn to propose the actionable information for different robotic manipulation primitives (\eg \textit{pushing}, \textit{pulling}): (a) the predicted actionability scores over pixels; (b) the proposed interaction trajectories along with their confident scores for a selected pixel highlighted in red.}}
    \label{fig:teaser}
    \vspace{-4mm}
\end{figure}


% high-level intro (the microwave example) 
3D objects, especially man-made ones, have rich interaction-oriented semantics and functionality, often highly localized to certain object parts and regions.
%
% There are rich interaction-oriented semantics and functionalities on 3D objects, especially for man-made ones, and many are highly coupled with certain object parts and regions.
%
For example, to operate a microwave for heating a cup of milk, one first need to locate and push the door button expecting the door to pop out.
If the door is not fully open, one then has to pull out the door by clamping the door edge and rotating the door to open to a larger degree.
Next, one places the cup with the milk at the center of the tray, closes the door, and sets up a timer by rotating the control knob on the side.
%
All these steps require perceiving and interacting with multiple parts of the microwave, using different types of interaction.


% high-level intro (parts, articulated objects / why the problem is interesting and challenging)
We humans demonstrate strong capabilities in perceiving and interacting with daily-life objects in the 3D world, by understanding object parts, functionalities and affordances.
%
However, this remains a complicated task for home-assistant robots to achieve, since it involves many challenging subtasks in computer vision and robotics, such as part detection, part motion estimation, and robotic actuation/manipulation.
%
For manipulating 3D articulated objects, robot agents need to learn perceive and detect these local ``active sites'' that are associated with specific actions/interactions on 3D object parts and the causal object state chances that can ensue by performing such actions.

\kaichun{TODO: add our usage demo: Assume object mask, part mask/seg, part motion are done by previous works; show some system-design where our new module is integrated and will be useful}

\kaichun{TODO: why learn perception from simulation? How it helps real-world RL learning: we can do random-exploration on synthetic data in simulation, hope this knowledge generalizes to real-world, so that it speeds up the exploration when training real-world RL policies
We can also collect some real-world data to finetune this backbone}


% state-of-the-art / previous works (perception & interaction)
Previous works in the computer vision community studied the problems of shape part segmentation~\cite{}, part motion estimation~\cite{}, and shape affordances~\cite{}.
%
However, most of these works stand purely on the vision side, learning no direct interaction-oriented information (such as affordances), or take a passive learning approach assuming the availability the ground-truth data with human functionality annotations, an approach that is not scalable to large-scale machine learning.
%
Robotic researchers investigated \kaichun{todo: part-aware/articulated object manipulation works.}
%
These works usually focus on learning downstream manipulation control policies and often demonstrate results over a limited number of shapes.
%
There is a recent trend on bridging the loop between perception and interaction that try to simultaneously learn visual representations and interaction skills~\cite{}, or interactive perception~\cite{}.


% in our paper, we formulate/propose a new task; why this formulation?
In this paper, we formulate a new task of inferring visual "actionable information" for manipulating 3D articulated objects.
%
Given an input 3D shape represented by a single image or a partial point cloud scan, we want to propose potential interaction types and parameters for every pixel, which leads to some object part motions and object state changes in a very short period of time.
%
%We consider six types of primitive interaction types: pushing, pushing-up, pushing-left, pulling, pulling-up, pulling-left, which are all parameterized in a space of 6-DoF robot gripper end-effector pose in SE(3) space.
%
In the context of robotic manipulation, we argue that such visual “actionable information” lies in the middle between the raw visual inputs to the final robotic manipulation task and helps bridge the gap between perception and interaction.
%
It learns an interaction-oriented visual representations that enjoys fast inference that generates visual predictions based on raw visual inputs and provides high-recall action proposals for downstream manipulation tasks at the same time.






% our method
To address this challenging problem, we propose a multi-head neural network architecture that has one backbone network for extracting per-pixel feature and three decoding modules that jointly predict the interaction proposals.
%
Taking as input an RGB image or a partial point cloud scan from a viewpoint, we first extract per-pixel/point feature adapting the standard encoder-decoder backbones with skip-connections.
%
Our network has three decoding heads: an actionability scoring module, an action proposal module and an action scoring module.
%
The actionability scoring module rates each pixel/point with an "actionability" score indicating whether a certain interaction type is applicable or not.
%
Then, for each actionable pixel/point, the action proposal module proposes high-recall interaction solutions, bearing the spirit of a conditional generative model, while the action scoring module predicts how much an interaction proposal will be successful.



% challenge (learn from interaction; hard-to-get-positive) and how to address challenges
We train the entire network by sampling interaction data in simulation, which free us from manual annotations for the training.
%
However, for naive random data sampling, it is highly unlikely for a random interaction on a random position to be successful. 
%
In other words, we have a severe data imbalance problem that only 1-3\% of sampled interaction trials are positive for the interaction types involving grasping, such as pulling.
%
We thus propose an on-policy data sampling strategy to alleviate this issue by sampling more datapoints over regions that the networks predicts to be positive.
%
We find that this strategy not only helps increase the sampling efficiency for positive interaction trials, but also help increase the final model performance.


% results and analysis
We use SAPIEN~\cite{chang2015shapenet,mo2019partnet,xiang2020sapien} as our main testbed, on which we create simulation environments and benchmarks for six types of primitive interaction, covering 989 shapes over 15 commonly seen indoor object categories. 
%
Experiments show that our method successfully learns such visual "actionable information" and beat the baseline methods.
%
More interestingly, we find that our network learns mostly local-context knowledges relevant to each of primitive interaction types which generalizes well to the unseen testing categories.
%
Finally, we demonstrate that our learned knowledge in SAPIEN simulator can transfer to real-world scenes from the \kaichun{REplica} dataset, as shown in Figure~\ref{fig:teaser} (b).


% final paragraph
In summary, our contributions are:
\begin{itemize}
    \vspace{-2mm}
    \item we formulate a novel challenging task of inferring visual affordance for manipulating 3D articulated objects;
    \vspace{-2mm}
    \item we propose an effective approach to tackle this problem;
    \vspace{-2mm}
    \item we create a benchmark using SAPIEN~\cite{xiang2020sapien} and demonstrate our superior performances on six types of interactions;
    \vspace{-2mm}
    \item we show that the learned knowledge in simulation successfully transfer to real-world data.
\end{itemize}




